CG-HAF: An Interpretable Global-Local Lesion-Burden Fusion Framework for Ordinal Acne Severity Grading in Agentic Skincare Support

Ordinal acne severity grading requires distinguishing visually similar neighboring grades while jointly weighing holistic facial appearance and localized lesion burden - evidence that most existing approaches collapse into a single opaque representation. We introduce CG-HAF, a global-local fusion framework that instead keeps this evidence explicit: averaged holistic severity probabilities from independently trained classifiers are combined with structured lesion-burden descriptors from an object detector (lesion count, detection confidence, lesion area) into a compact representation, from which a lightweight, interpretable classifier produces the final grade. On a widely used benchmark, this fusion yields a clear, statistically supported improvement over global-evidence-only baselines, with the largest gains on the most severe cases. Testing on an independent dataset with a different grading standard shows that strong within-dataset performance does not transfer automatically, and a follow-up diagnostic attributes much of this gap to mismatched grading criteria rather than detection failure alone. These findings support interpretable global-local fusion as an effective strategy for ordinal acne grading while highlighting criterion alignment as key to cross-dataset portability, with a further illustration of how the resulting severity signal can support transparent, non-diagnostic decision-making in skincare applications.

==> author_audits/introduction_audit.tex <==
% AUTHOR-ONLY MATERIAL -- DO NOT INCLUDE IN SUBMISSION-FACING main.tex
% This file preserves the audit material contained in the source DOCX.
% Required packages if compiled separately: longtable, pdflscape, array

\section*{Citation Traceability Audit --- remove before manuscript submission}
Audit note: PDF line numbers are not stable in the extracted corpus, so exact PDF pages, section labels, paragraph openings, and short source fragments are reported instead. Selected bibliographic records were independently checked against publisher/proceedings metadata where available.

\begin{landscape}
\tiny
\setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1.08}
\begin{longtable}{|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|}
\hline
\textbf{Sentence ID} & \textbf{Exact manuscript sentence} & \textbf{Citation number(s)} & \textbf{Exact paper title} & \textbf{Exact PDF page} & \textbf{Relevant paper section/subsection} & \textbf{Extracted line range if available} & \textbf{If lines are unavailable, paragraph opening words} & \textbf{Supporting source fragment, maximum 15 words} & \textbf{Support type} & \textbf{Notes on inference or limitations} & \textbf{Verification status} \\ \hline
\endfirsthead
\hline
\textbf{Sentence ID} & \textbf{Exact manuscript sentence} & \textbf{Citation number(s)} & \textbf{Exact paper title} & \textbf{Exact PDF page} & \textbf{Relevant paper section/subsection} & \textbf{Extracted line range if available} & \textbf{If lines are unavailable, paragraph opening words} & \textbf{Supporting source fragment, maximum 15 words} & \textbf{Support type} & \textbf{Notes on inference or limitations} & \textbf{Verification status} \\ \hline
\endhead
P1-S2 & The ACNE04 study formalized this setting by pairing facial images with both lesion-count information and four severity grades, and it highlighted that cases with neighboring severities can exhibit similar appearance [1]. & [1] & Joint Acne Image Grading and Counting via Label Distribution Learning & 1--2 & Abstract; Introduction & N/A --- PDF extraction has no stable line numbering & ``Accurate grading of skin disease severity...'' & ``appearance similarity of acne with close severity'' & paraphrase & Supports ACNE04, neighboring-grade ambiguity, and LDL motivation. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P1-S3 & A recent systematic review likewise characterizes conventional acne assessment as relying mainly on global severity grading and lesion counting, with each approach offering complementary information but also introducing subjectivity or practical burden [2]. & [2] & Artificial Intelligence in the Assessment and Grading of Acne Vulgaris: A Systematic Review & 2; 9--11 & Introduction; Discussion/Conclusions & N/A --- PDF extraction has no stable line numbering & ``Traditional acne-severity assessment tools...'' & ``global acne severity grading and lesion counting'' & paraphrase & Supports complementary assessment modes, imbalance, and external-validation limitations. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P1-S5 & Label-distribution formulations have therefore been used to model ambiguity near grade boundaries rather than treating each image as belonging to an isolated class with no neighborhood structure [1], [3]. & [1] & Joint Acne Image Grading and Counting via Label Distribution Learning & 1--2 & Abstract; Introduction & N/A --- PDF extraction has no stable line numbering & ``Accurate grading of skin disease severity...'' & ``appearance similarity of acne with close severity'' & synthesis & Supports ACNE04, neighboring-grade ambiguity, and LDL motivation. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P1-S5 & Label-distribution formulations have therefore been used to model ambiguity near grade boundaries rather than treating each image as belonging to an isolated class with no neighborhood structure [1], [3]. & [3] & Improving Acne Image Grading with Label Distribution Smoothing & 1--2 & Abstract; Introduction & N/A --- PDF extraction has no stable line numbering & ``Acne severity grading typically involves...'' & ``manage label uncertainty without compromising class distinctiveness'' & synthesis & Uploaded PDF is arXiv v1; bibliographic record normalized to peer-reviewed ISBI 2024. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P2-S2 & Global image-level models can learn holistic cues such as facial erythema, texture, overall lesion distribution, and broad severity patterns, while global--local architectures such as KIEGLFN show that local skin information can complement whole-face representations [4]. & [4] & KIEGLFN: A unified acne grading framework on face images & 1--3 & Abstract; Introduction; Global Local Fusion Network & N/A --- PDF extraction has no stable line numbering & ``Grading the severity level is...'' & ``fuses global deep features with local features'' & methodological positioning & Supports explicit global--local motivation and architecture. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P2-S3 & Diagnostic Evidence Distillation similarly emphasizes that the type and number of fine-grained lesions constitute severity-relevant evidence, but its final student model is designed to infer severity from the facial image after lesion evidence has been used for training-time guidance [5]. & [5] & DED: Diagnostic Evidence Distillation for acne severity grading on face images & 1; 4 & Abstract; Introduction & N/A --- PDF extraction has no stable line numbering & ``Acne seriously affects people's daily life...'' & ``student model learns ... from only face images'' & methodological positioning & Supports use of lesion evidence as training-time guidance and image-only final student inference. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P2-S4 & In contrast, detector- and count-centered pipelines make local evidence explicit: AcneDet detects lesion types and passes their counts to a downstream grading model, yielding a comparatively transparent count-to-grade pathway [6], while interpretable object-detection models can localize lesions and derive severity estimates from the resulting detections [7]. & [6] & Automatic Acne Object Detection and Acne Severity Grading Using Smartphone Images and Artificial Intelligence & 1; 5; 10 & Abstract; Methods; Discussion & N/A --- PDF extraction has no stable line numbering & ``Skin image analysis using artificial intelligence...'' & ``counts of each acne type ... used as input'' & synthesis & Supports explicit detector-to-count grading and higher-grade imbalance. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P2-S4 & In contrast, detector- and count-centered pipelines make local evidence explicit: AcneDet detects lesion types and passes their counts to a downstream grading model, yielding a comparatively transparent count-to-grade pathway [6], while interpretable object-detection models can localize lesions and derive severity estimates from the resulting detections [7]. & [7] & Acne detection and severity evaluation with interpretable convolutional neural network models & 1 & Abstract & N/A --- PDF extraction has no stable line numbering & ``BACKGROUND: Acne vulgaris is...'' & ``object detection models ... better interpretability'' & synthesis & Supports localized, interpretable detection-derived severity assessment. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P2-S5 & Local analysis is itself difficult, however, because acne lesions may be small, densely distributed, and affected by illumination and scale variation [8]. & [8] & ACNet: Mask-Aware Attention with Dynamic Context Enhancement for Robust Acne Detection & 1 & Abstract; Introduction & N/A --- PDF extraction has no stable line numbering & ``Computer-aided diagnosis has recently received...'' & ``color shift ... variation in scales ... high density'' & methodological positioning & Supports technical difficulty of local acne detection. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P2-S6 & Moreover, datasets can be strongly imbalanced at higher grades, and minority Severe or Very-Severe cases may be obscured by aggregate metrics [2], [6]. & [2] & Artificial Intelligence in the Assessment and Grading of Acne Vulgaris: A Systematic Review & 2; 9--11 & Introduction; Discussion/Conclusions & N/A --- PDF extraction has no stable line numbering & ``Traditional acne-severity assessment tools...'' & ``global acne severity grading and lesion counting'' & synthesis & Supports complementary assessment modes, imbalance, and external-validation limitations. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P2-S6 & Moreover, datasets can be strongly imbalanced at higher grades, and minority Severe or Very-Severe cases may be obscured by aggregate metrics [2], [6]. & [6] & Automatic Acne Object Detection and Acne Severity Grading Using Smartphone Images and Artificial Intelligence & 1; 5; 10 & Abstract; Methods; Discussion & N/A --- PDF extraction has no stable line numbering & ``Skin image analysis using artificial intelligence...'' & ``counts of each acne type ... used as input'' & synthesis & Supports explicit detector-to-count grading and higher-grade imbalance. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P3-S2 & Ordinal ambiguity has been modeled through label distribution learning and severity-aware label smoothing [1], [3]. & [1] & Joint Acne Image Grading and Counting via Label Distribution Learning & 1--2 & Abstract; Introduction & N/A --- PDF extraction has no stable line numbering & ``Accurate grading of skin disease severity...'' & ``appearance similarity of acne with close severity'' & synthesis & Supports ACNE04, neighboring-grade ambiguity, and LDL motivation. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P3-S2 & Ordinal ambiguity has been modeled through label distribution learning and severity-aware label smoothing [1], [3]. & [3] & Improving Acne Image Grading with Label Distribution Smoothing & 1--2 & Abstract; Introduction & N/A --- PDF extraction has no stable line numbering & ``Acne severity grading typically involves...'' & ``manage label uncertainty without compromising class distinctiveness'' & synthesis & Uploaded PDF is arXiv v1; bibliographic record normalized to peer-reviewed ISBI 2024. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P3-S3 & Ensemble methods such as AcneGrader combine multiple image classifiers to improve grading robustness at the cost of a larger collection of base models [9]. & [9] & AcneGrader: An ensemble pruning of the deep learning base models to grade acne & 1; 11--12 & Abstract; Discussion & N/A --- PDF extraction has no stable line numbering & ``Background: Acne is one of...'' & ``ensemble pruning strategy ... removing the redundant base models'' & methodological positioning & Supports ensemble robustness/computational complexity positioning. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P3-S4 & Global--local methods explicitly combine whole-face and local visual representations [4], while prior-knowledge-guided approaches inject lesion-related information into the grading process [10]. & [4] & KIEGLFN: A unified acne grading framework on face images & 1--3 & Abstract; Introduction; Global Local Fusion Network & N/A --- PDF extraction has no stable line numbering & ``Grading the severity level is...'' & ``fuses global deep features with local features'' & synthesis & Supports explicit global--local motivation and architecture. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P3-S4 & Global--local methods explicitly combine whole-face and local visual representations [4], while prior-knowledge-guided approaches inject lesion-related information into the grading process [10]. & [10] & Acne Severity Grading on Face Images via Extraction and Guidance of Prior Knowledge & 1--2 & Abstract; Introduction & N/A --- PDF extraction has no stable line numbering & ``Acne Vulgaris seriously affects...'' & ``number and type of small objects are the evidence'' & synthesis & Supports prior-knowledge injection for grading. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P3-S5 & Evidence-distillation and feature-feedback methods further transfer or refine task-relevant information during training [5], [11]. & [5] & DED: Diagnostic Evidence Distillation for acne severity grading on face images & 1; 4 & Abstract; Introduction & N/A --- PDF extraction has no stable line numbering & ``Acne seriously affects people's daily life...'' & ``student model learns ... from only face images'' & synthesis & Supports use of lesion evidence as training-time guidance and image-only final student inference. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P3-S5 & Evidence-distillation and feature-feedback methods further transfer or refine task-relevant information during training [5], [11]. & [11] & Feature Feedback-Based Pseudo-Label Learning for Multi-Standards in Clinical Acne Grading & 1--2 & Abstract; Introduction & N/A --- PDF extraction has no stable line numbering & ``Accurate acne grading is critical...'' & ``feature feedback ... iterative pseudo-label refinement'' & synthesis & Supports feature-feedback training strategy; no claim of superiority is imported. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P3-S6 & Lesion-centric systems estimate severity from detected or segmented lesions and their derived counts or scores [6], [12]. & [6] & Automatic Acne Object Detection and Acne Severity Grading Using Smartphone Images and Artificial Intelligence & 1; 5; 10 & Abstract; Methods; Discussion & N/A --- PDF extraction has no stable line numbering & ``Skin image analysis using artificial intelligence...'' & ``counts of each acne type ... used as input'' & synthesis & Supports explicit detector-to-count grading and higher-grade imbalance. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P3-S6 & Lesion-centric systems estimate severity from detected or segmented lesions and their derived counts or scores [6], [12]. & [12] & AcneAI: A New Acne Severity Assessment Method Using Digital Images and Deep Learning & 1--3 & Abstract; Introduction; Method & N/A --- PDF extraction has no stable line numbering & ``In this paper we present...'' & ``combining individual acne lesion scores into an overall'' & synthesis & Uploaded manuscript normalized to published MICCAI 2024 chapter. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P3-S7 & Recent controlled studies also reinforce that subtle localized cues and ordinal relationships require evaluation beyond generic representation quality [13]. & [13] & A Study of SimCLR-Based Self-Supervised Learning for Acne Severity Grading Under Label-Scarce Conditions & 1--2; 8 & Abstract; Introduction; Evaluation Metrics & N/A --- PDF extraction has no stable line numbering & ``Acne severity grading is an important...'' & ``subtle, localized features and ordinal relationships'' & methodological positioning & Supports need for ordinal and localized-cue-aware evaluation. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P3-S8 & Comparative acne-classification studies continue to show substantial methodological variation across architectures and grading protocols [14]. & [14] & An experimental evaluation of deep learning-based models for acne severity classification in humans & 2--4 & Abstract; Introduction; Related Work & N/A --- PDF extraction has no stable line numbering & ``Acne is a chronic inflammatory...'' & ``comparative analysis ... for acne severity classification'' & methodological positioning & Supports continuing architectural/protocol variation in recent acne classification studies. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
P3-S9 & More broadly, the acne-AI literature remains dominated by retrospective internal evaluation, with limited external validation and incomplete reporting of population diversity or real-world generalization [2]. & [2] & Artificial Intelligence in the Assessment and Grading of Acne Vulgaris: A Systematic Review & 2; 9--11 & Introduction; Discussion/Conclusions & N/A --- PDF extraction has no stable line numbering & ``Traditional acne-severity assessment tools...'' & ``global acne severity grading and lesion counting'' & methodological positioning & Supports complementary assessment modes, imbalance, and external-validation limitations. & Verified against uploaded full text; bibliography independently checked for selected reference \\ \hline
\end{longtable}
\end{landscape}


\section*{Introduction Literature Selection Audit --- remove before manuscript submission}
Screening basis: all 150 supplied PDFs were text-extracted and screened across their full available content. Papers with direct acne-grading, lesion-detection, ordinal-learning, fusion, or reliability relevance were then examined in their substantive sections (Introduction/Methods/Results/Discussion/Conclusion as applicable). ``DO NOT SELECT'' means not selected for this Introduction and does not preclude later use in Related Work.

\begin{landscape}
\tiny
\setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1.08}
\begin{longtable}{|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|}
\hline
\textbf{Uploaded filename} & \textbf{Exact paper title} & \textbf{Year} & \textbf{Venue} & \textbf{DOI/publication identifier} & \textbf{Main research topic} & \textbf{Relevance to CG-HAF Introduction} & \textbf{Relevance level} & \textbf{Specific Introduction claim it could support} & \textbf{Duplicate/superseded status} & \textbf{Final Introduction decision} & \textbf{Reason} \\ \hline
\endfirsthead
\hline
\textbf{Uploaded filename} & \textbf{Exact paper title} & \textbf{Year} & \textbf{Venue} & \textbf{DOI/publication identifier} & \textbf{Main research topic} & \textbf{Relevance to CG-HAF Introduction} & \textbf{Relevance level} & \textbf{Specific Introduction claim it could support} & \textbf{Duplicate/superseded status} & \textbf{Final Introduction decision} & \textbf{Reason} \\ \hline
\endhead
DEDDiagnosticEvidenceDistillationforacneseveritygradingonfaceimages.pdf & DED: Diagnostic Evidence Distillation for acne severity grading on face images & 2023 & Expert Systems with Applications & 10.1016/j.eswa.2023.120312 & Acne severity grading / lesion-aware assessment & Directly relevant to ordinal grading, lesion burden, or evaluation. & Core & Diagnostic-evidence distillation and training-time lesion evidence & None identified & SELECT & Directly supports a necessary Introduction claim; retained after full-text review and bibliographic verification. \\ \hline
[100]Dan\_TransFace\_Calibrating\_Transformer\_Training\_for\_Face\_Recognition\_from\_a\_Data-Centric\_ICCV\_2023\_paper.pdf & TransFace: Calibrating Transformer Training for Face Recognition from a Data-Centric Perspective & Not independently verified & IEEE International Conference on Computer Vision & Not independently verified (not selected) & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[101]Deciphering\_Consumer\_Skin\_Care\_Needs\_Analyzing\_Sentiments\_and\_Review\_Topics\_of\_Cetaphil\_Facial\_Wash\_Across\_Diverse\_Skin\_Types.pdf & Deciphering Consumer Skin Care Needs: Analyzing Sentiments and Review Topics of Cetaphil Facial Wash Across Diverse Skin Types & 2023 & 2023 International Conference on Information Technology and Computing (ICITCOM) & 10.1109/ICITCOM60176.2023.10442129 & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[102]Deep\_Learning-Based\_Skin\_type\_Classification\_using\_Fine-Tuned\_ResNet50\_Architecture.pdf & Deep Learning-Based Skin type Classification using Fine-Tuned ResNet50 Architecture & 2025 & 2025 International Conference on Intelligent and Innovative Technologies in Computing, Electrical and Electronics (IITCEE) & 10.1109/IITCEE64140.2025.10915335 & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[103]FaceSkin\_A\_Privacy\_Preserving\_Facial\_skin\_patch\_Dataset\_for\_multi\_Attributes\_classification.pdf & FaceSkin: A Privacy Preserving Facial skin patch Dataset for multi Attributes classification & 2023 & 2023 International Conference on Image Processing, Computer Vision and Machine Learning (ICICML) & 10.1109/ICICML60161.2023.10424824 & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[104]Semi-Supervised\_Skin\_Lesion\_Segmentation\_With\_Coupling\_CNN\_and\_Transformer\_Features.pdf & Semi-Supervised Skin Lesion Segmentation With Coupling CNN and Transformer Features & 2022 & IEEE Access & 10.1109/ACCESS.2022.3224005 & Dermatology AI / skin-image analysis & Provides broad reliability or medical-image context but is not acne-grading specific. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[104]facial-recognition-nytimes.pdf & Facial Recognition Is Accurate, if You're a White Guy - The New York Times & 2018 & Not independently verified (not selected) & Not independently verified (not selected) & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[105]FacialSkinTypeClassificationBasedonMicroscopic.pdf & Facial Skin Type Classification Based on Microscopic Images using Convolutional Neural Network (CNN) & 2020 & Not independently verified (not selected) & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[106]Feature\_Extraction\_for\_Facial\_Skin\_Type\_Classification\_Using\_Photo\_Images.pdf & Feature Extraction for Facial Skin Type Classification Using Photo Images & 2024 & 2024 9th International Conference on Information Technology and Digital Applications (ICITDA) & 10.1109/ICITDA64560.2024.10809552 & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[107]paper3.pdf & Wrinkle Image Classification Using CNN (title not recoverable beyond schematic/text in supplied PDF) & 2023 & Not independently verified (not selected) & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[108]2203.16056v1.pdf & Automatic Facial Skin Feature Detection for Everyone & 2022 & Not independently verified (not selected) & arXiv:2203.16056v1 & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[109]Combining Diamond-Tip Dermabrasion Treatments and Topical Skincare in Participants with Dry  Hyperpigmented  Photodamaged or Acne-Prone Oily Facial Sk.pdf & Combining Diamond-Tip Dermabrasion Treatments and Topical Skincare in Participants with Dry, Hyperpi & 2023 & gy   ISSN: 1178-7015 (Online) Journal homepage: www.tandfonline.com/journals/dcci20   Combining Diamond-Tip Dermabrasion   Treatments and Topical Skincare in Pa & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[10]2308.08155v2.pdf & AutoGen: Enabling Next-Gen LLM Applications via Multi-Agent Conversation & 2023 & Not independently verified (not selected) & arXiv:2308.08155v2 & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[110]cosmetics-10-00041-v3.pdf & 3D Printed Hollow Microneedles for Treating Skin Wrinkles Using Different Anti-Wrinkle Agents: A Possible Futuristic Approach & 2023 & Not independently verified (not selected) & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[111]cosmetics-12-00125.pdf & The Effectiveness of a Topical Rosehip Oil Treatment on Facial Skin Characteristics: A Pilot Study on Wrinkles, UV Spots Reduction, Erythema Mitigation, and Age-Related Signs & 2025 & Not independently verified (not selected) & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[112]diagnostics-13-01894.pdf & Deep-Learning-Based Morphological Feature Segmentation for Facial Skin Image Analysis & 2023 & diagnostics   Article   Deep-Learning-Based Morphological Feature Segmentation for   Facial Skin Image Analysis   Huisu Yoon *, Semin Kim , Jongha Lee and Sangw & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[113]Effects-of-wrinkle-treatments-on-hyperpigmentation-in-high-uv-index-enviroment-Balserio.pdf & Effects of Wrinkle Treatment on Facial Hyperpigmentation in a High UV Environment & 2024 & Not independently verified (not selected) & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[114]electronics-11-03623-v2.pdf & Classifying Conditions of Speckle and Wrinkle on the Human Face: A Deep Learning Approach & 2022 & electronics   Article   Classifying Conditions of Speckle and Wrinkle on the Human   Face: A Deep Learning Approach   Tsai-Rong Chang * and Ming-Yen Tsai   Depa & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[115]electronics-12-04897.pdf & Facial Wrinkle Detection with Multiscale Spatial Feature Fusion Based on Image Enhancement and ASFF-SEUnet & 2023 & electronics   Article   Facial Wrinkle Detection with Multiscale Spatial Feature Fusion   Based on Image Enhancement and ASFF-SEUnet   Jiang Chen 1 , Mingfang H & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[116]healthcare-10-02396.pdf & An Optimization-Based Technology Applied for Face Skin Symptom Detection & 2022 & Not independently verified (not selected) & Not independently verified (not selected) & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & Exact duplicate pair with [60]healthcare-10-02396.pdf & DO NOT SELECT & Redundant duplicate; not needed for Introduction. \\ \hline
[117]I4.006.pdf & Facial Skin Texture and Distributed Dynamic Kernel Support Vector Machine (DDKSVM) Classifier for Age Estimation in Facial Wrinkles & 2023 & Not independently verified (not selected) & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[118]ijms-26-10022.pdf & Microbiome--Aging--Wrinkles Axis of Skin: Molecular Insights and Microbial Interventions & 2025 & Not independently verified (not selected) & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[119]J of Cosmetic Dermatology - 2024 - He - Dendrobium officinale flowers  topical extracts improve skin oxidative stress and.pdf & Dendrobium officinale flowers' topical extracts improve skin oxidative stress and aging & 2024 & J of Cosmetic Dermatology 2024.23:1891-1904 & 10.1111/jocd.16210 & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[11]2308.11432v7.pdf & A Survey on Large Language Model based Autonomous Agents & 2025 & Front. Comput. Sci., 2025, 0(0): 1--42   https://doi.org/10.1007/s11704-024-40231-1   REVIEW ARTICLE   A Survey on Large Language Model based Autonomous   Agents & arXiv:2308.11432v7 & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[120]J of Cosmetic Dermatology - 2025 - Zhao - Noninvasive Assessment Methods for the Therapeutic Effect Following Facial.pdf & Noninvasive Assessment Methods for the Therapeutic Effect Following Facial Rejuvenation & 2025 & J of Cosmetic Dermatology 2025.24:e70482 & Not independently verified (not selected) & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[121]JHEP10(2023)069.pdf & Wrinkles in the Froggatt-Nielsen mechanism and flavorful new physics & 2023 & Not independently verified (not selected) & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[122]s40820-023-01252-w.pdf & Highly Thermoconductive, Strong Graphene-Based Composite Films by Eliminating Nanosheets Wrinkles & 2024 & Nano-Micro Letters, https://doi.org/10.1007/s40820-023-01252-w & 10.1007/s40820-023-01252-w & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[123]s41377-023-01285-1.pdf & Voxelated opto-physically unclonable functions via irreplicable wrinkles & 2023 & Light: Science \& Applications, doi:10.1038/s41377-023-01285-1 & 10.1038/s41377-023-01285-1 & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[124]s41467-022-31887-z.pdf & Large-area transfer of two-dimensional materials free of cracks, contamination and wrinkles via controllable conformal contact & 2022 & Nature Communications, doi:10.1038/s41467-022-31887-z & 10.1038/s41467-022-31887-z & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[125]Sanchez\_ACCVW\_Phot.pdf & Photorealistic Facial Wrinkles Removal & 2025 & Asian Conference on Computer Vision Workshops & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[126]Skin Research and Technology - 2023 - Carlos da Silva - Detection of skin wrinkles and quantification of roughness using a.pdf & Detection of skin wrinkles and quantification of roughness using a novel image processing technique from a dermatoscope device & 2023 & Not independently verified (not selected) & 10.1111/srt.13335 & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[127]The Characteristics of the Skin Physiological Parameters and Facial Microbiome of  Ideal Skin  in Shanghai Women.pdf & The Characteristics of the Skin Physiological Parameters and Facial Microbiome of ``Ideal Skin'' in Sh & 2023 & gy   ISSN: 1178-7015 (Online) Journal homepage: www.tandfonline.com/journals/dcci20   The Characteristics of the Skin Physiological   Parameters and Facial Micr & Not independently verified (not selected) & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[128]toxins-14-00342-v2.pdf & Novel Anatomical Guidelines on Botulinum Neurotoxin Injection for Wrinkles in the Nose Region & 2022 & Not independently verified (not selected) & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[129]1-s2.0-S0010482523008788-main.pdf & Artificial intelligence-assisted dermatology diagnosis: From unimodal to multimodal & 2023 & Computers in Biology and Medicine, 165 (2023) 107413. doi:10.1016/j.compbiomed.2023.107413 & 10.1016/j.compbiomed.2023.107413 & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[12]2309.07864v3.pdf & The Rise and Potential of Large Language Model Based Agents: A Survey & 2023 & Not independently verified (not selected) & arXiv:2309.07864v3 & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[130]1-s2.0-S2352914823001570-main.pdf & AI-assisted mole detection for online dermatology triage in telemedicine settings & 2023 & Informatics in Medicine Unlocked, 41 (2023) 101311. doi:10.1016/j.imu.2023.101311 & 10.1016/j.imu.2023.101311 & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[131]Acad Dermatol Venereol - 2023 - Sangers - Position statement of the EADV Artificial Intelligence  AI  Task Force on.pdf & Position statement of the EADV Artificial Intelligence (AI) Task Force on AI‐assisted smartphone apps and web‐based services for skin disease & 2024 & Acad Dermatol Venereol 2024.38:22-30 & 10.1111/jdv.19521 & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[132]applsci-15-07856.pdf & Artificial Intelligence in Dermatology: A Review of Methods, Clinical Applications, and Perspectives & 2016 & Not independently verified (not selected) & Not independently verified (not selected) & Dermatology AI / skin-image analysis & Provides broad reliability or medical-image context but is not acne-grading specific. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[133]Artificial\_Intelligence\_in\_Cosmetic\_Dermatology\_A\_Systematic\_Literature\_Review.pdf & Artificial Intelligence in Cosmetic Dermatology: A Systematic Literature Review & 2023 & IEEE Access & 10.1109/ACCESS.2023.3295001 & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[134]e050203.full.pdf & Improving Skin cancer Management with ARTificial Intelligence (SMARTI): protocol for a preintervention/postintervention trial of an artificial intelligence system used as a diagnostic aid for skin cancer management in a specialist dermatology setting & 2021 & Open access Protocol   BMJ Open: first published as 10.1136/bmjopen-2021-050203 on 4 January 2022. Downloaded from http://bmjopen.bmj.com/ on February 8, 2026 & Not independently verified (not selected) & Dermatology AI / skin-image analysis & Provides broad reliability or medical-image context but is not acne-grading specific. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[135]fmed-10-1278232.pdf & Principles, applications, and future of artificial intelligence in dermatology & 2023 & ﻿This paper provides an overview of artificial-intelligence (AI), as applied to dermatology. & 10.3389/fmed.2023.1278232 & Dermatology AI / skin-image analysis & Provides broad reliability or medical-image context but is not acne-grading specific. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[136]Int J Dermatology - 2024 - Fliorent - Artificial intelligence in dermatology  advancements and challenges in skin of color.pdf & Artificial intelligence in dermatology: advancements and challenges in skin of color & 2024 & Int J Dermatology 2024.63:455-461 & Not independently verified (not selected) & Dermatology AI / skin-image analysis & Provides broad reliability or medical-image context but is not acne-grading specific. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[137]J of Cosmetic Dermatology - 2024 - Kania - Artificial intelligence in cosmetic dermatology.pdf & Artificial intelligence in cosmetic dermatology & 2024 & J of Cosmetic Dermatology 2024.23:3305-3311 & 10.1111/jocd.16538 & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[138]J of Cosmetic Dermatology - 2024 - Thunga - AI in Aesthetic Cosmetic Dermatology  Current and Future.pdf & AI in Aesthetic/Cosmetic Dermatology: Current and Future & 2025 & J of Cosmetic Dermatology 2025.24:e16640 & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[139]J of Cosmetic Dermatology - 2025 - Haykal - Advances in Longevity  The Intersection of Regenerative Medicine and Cosmetic.pdf & Advances in Longevity: The Intersection of Regenerative Medicine and Cosmetic Dermatology & 2025 & J of Cosmetic Dermatology 2025.24:e70356 & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[13]2309.10062v2.pdf & SMART-LLM: Smart Multi-Agent Robot Task Planning using Large Language Models & 2024 & Not independently verified (not selected) & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[140]jcm-11-06826-v4.pdf & Artificial Intelligence in Dermatology Image Analysis: Current Developments and Future Trends & 2022 & Journal of   Clinical Medicine   Review   Artificial Intelligence in Dermatology Image Analysis: Current   Developments and Future Trends   Zhouxiao Li 1,2,† , & Not independently verified (not selected) & Dermatology AI / skin-image analysis & Provides broad reliability or medical-image context but is not acne-grading specific. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[141]JSIAR-M-25-05800.pdf & Smart Dermatology: Revolutionizing Skincare with AI-Driven CNN-Based Detection and Product Recommendation System & 2025 & Not independently verified (not selected) & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[142]s13555-022-00833-8.pdf & Artificial Intelligence in Dermatology: Challenges and Perspectives & 2022 & Dermatology and Therapy, https://doi.org/10.1007/s13555-022-00833-8 & 10.1007/s13555-022-00833-8 & Dermatology AI / skin-image analysis & Provides broad reliability or medical-image context but is not acne-grading specific. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[143]-M-Acne\_Severity\_Grading\_on\_Face\_Images\_via\_Extraction\_and\_Guidance\_of\_Prior\_Knowledge.pdf & Acne Severity Grading on Face Images via Extraction and Guidance of Prior Knowledge & 2022 & 2022 IEEE International Conference on Bioinformatics and Biomedicine (BIBM) & 10.1109/BIBM55620.2022.9995101 & Acne severity grading / lesion-aware assessment & Directly relevant to ordinal grading, lesion burden, or evaluation. & Core & Prior-knowledge extraction/guidance from lesion evidence & None identified & SELECT & Directly supports a necessary Introduction claim; retained after full-text review and bibliographic verification. \\ \hline
[144]1604.02878v1.pdf & Joint Face Detection and Alignment using Multi-task Cascaded Convolutional Networks & 2016 & IEEE Transactions on Magnetics & Not independently verified (not selected) & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[145]-M-Automatic\_acne\_detection\_model\_based\_on\_improved\_Y.pdf & Automatic acne detection model based on improved YOLOv7 & 2024 & IEEE Access & 10.1109/ACCESS.2024.3520641 & Acne lesion detection/localization & Relevant to the local lesion-evidence branch and detection challenges. & Strongly relevant & Alternative acne grading/detection evidence; reserve for deeper Related Work comparison. & Author/prepublication version; superseded by final IEEE Access file [64]. & DO NOT SELECT & Superseded/prepublication version; prefer final published version where relevant. \\ \hline
[146]-M-ACNet\_Mask-Aware\_Attention\_with\_Dynamic\_Context\_Enhancement\_for\_Robust\_Acne\_Detection.pdf & ACNet: Mask-Aware Attention with Dynamic Context Enhancement for Robust Acne Detection & 2021 & 2021 IEEE International Conference on Systems, Man, and Cybernetics (SMC) & 10.1109/SMC52423.2021.9659243 & Acne lesion detection/localization & Relevant to the local lesion-evidence branch and detection challenges. & Core & Illumination, scale, small/dense-lesion detection challenges & None identified & SELECT & Directly supports a necessary Introduction claim; retained after full-text review and bibliographic verification. \\ \hline
[14]2401.00812v2.pdf & If LLM Is the Wizard, Then Code Is the Wand: A Survey on How Code Empowers Large Language Models to Serve as Intelligent Agents & 2024 & Not independently verified (not selected) & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[15]2403.03101v3.pdf & KnowAgent: Knowledge-Augmented Planning for LLM-Based Agents & 2025 & Not independently verified (not selected) & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[16]2404.04834v4.pdf & LLM-Based Multi-Agent Systems for Software Engineering: Literature Review, Vision and the Road Ahead & 2025 & -  Software and its engineering  ->  Software development techniques.Collaboration in software development. & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[17]2410.19855v1.pdf & Personalized Recommendation Systems using Multimodal, Autonomous, Multi Agent Systems & 2024 & Not independently verified (not selected) & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[18]2410.22457v1.pdf & Advancing Agentic Systems: Dynamic Task Decomposition, Tool Integration and Evaluation using Novel Metrics and Dataset & 2024 & Not independently verified (not selected) & arXiv:2410.22457v1 & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[19]2508.11957v1.pdf & A Comprehensive Review of AI Agents: Transforming Possibilities in Technology and Beyond & Not independently verified & Not independently verified (not selected) & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[1]Toward\_Data\_Systems\_That\_Are\_Business\_Semantic\_Centric\_and\_AI\_Agents\_Assisted.pdf & Toward Data Systems That Are Business Semantic Centric and AI Agents Assisted & 2025 & IEEE Access & 10.1109/ACCESS.2025.3583260 & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[20]2508.13843v1.pdf & UniECS: Unified Multimodal E-Commerce Search Framework with Gated Cross-modal Fusion & 2025 & -  Information systems  ->  Novelty in information retrieval.Similarity measures.Multimedia and multimodal retrieval. & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[21]2510.05759v3.pdf & OneVision: An End-to-End Generative Framework for Multi-view E-commerce Vision Search & 2025 & Not independently verified (not selected) & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[22]2511.14764v1.pdf & Image-Seeking Intent Prediction for Cross-Device Product Search & 2025 & Not independently verified (not selected) & Not independently verified (not selected) & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[23]6215\_Toolformer\_Language\_Model.pdf & Toolformer: Language Models Can Teach Themselves to Use Tools & 2023 & Not independently verified (not selected) & Not independently verified (not selected) & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[24]Agentic\_AI\_A\_Comprehensive\_Survey\_of\_Technologies\_Applications\_and\_Societal\_Implications.pdf & Agentic AI: A Comprehensive Survey of Technologies, Applications, and Societal Implications & 2025 & IEEE Access & 10.1109/ACCESS.2025.3585609 & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[25]Agentic\_AI\_Systems\_Architecture\_and\_Evaluation\_Using\_a\_Frictionless\_Parking\_Scenario.pdf & Agentic AI Systems: Architecture and Evaluation Using a Frictionless Parking Scenario & 2025 & IEEE Access & 10.1109/ACCESS.2025.3590264 & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[26]AIoT\_Smart\_Home\_via\_Autonomous\_LLM\_Agents.pdf & AIoT Smart Home via Autonomous LLM Agents & 2025 & IEEE Internet of Things Journal & 10.1109/JIOT.2024.3471904 & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[27]BFb0013570.pdf & Is It an Agent, or Just a Program?: A Taxonomy for Autonomous Agents & Not independently verified & Not independently verified (not selected) & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[28]Chatbot\_for\_E-Commerce\_Service\_Based\_on\_Rasa\_Framework\_and\_BERT\_Model.pdf & Chatbot for E-Commerce Service Based on Rasa Framework and BERT Model & 2024 & 2024 16th International Conference on Knowledge and System Engineering (KSE)   CHATBOT FOR E-COMMERCE SERVICE   BASED ON RASA FRAMEWORK AND   BERT MODEL   Truc & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[29]electronics-12-02722-v2.pdf & Emergent Cooperation and Strategy Adaptation in Multi-Agent Systems: An Extended Coevolutionary Theory with LLMs & 2023 & electronics   Article   Emergent Cooperation and Strategy Adaptation in Multi-Agent   Systems: An Extended Coevolutionary Theory with LLMs   I. de Zarzà 1,2,3 , & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[2]1703.02344v1.pdf & Deep Learning based Large Scale Visual Recommendation and Search for E-Commerce & 2017 & Not independently verified (not selected) & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[30]Enhancing\_E-commerce\_with\_Artificial\_Intelligence\_Applications\_for\_Better\_Customer\_Experience.pdf & Enhancing E-commerce with Artificial Intelligence Applications for Better Customer Experience & 2024 & 2024 5th International Conference on Communications, Information, Electronic and Energy Systems (CIEES) & 10.1109/CIEES62939.2024.10811370 & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[31]Genaiecom24\_paper\_10.pdf & Towards More Relevant Product Search Ranking Via  Large Language Models: An Empirical Study & 2024 & -  Computing methodologies  ->  Learning to rank.Ranking.Natural language processing. & Not independently verified (not selected) & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[32]Genaiecom24\_paper\_11.pdf & Hierarchical Knowledge Graph Construction from Images for Scalable E-Commerce & 2024 & -  Information systems  ->  Data mining. & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[33]Generative\_Agents\_in\_Agent-Based\_Modeling\_Overview\_Validation\_and\_Emerging\_Challenges.pdf & Generative Agents in Agent-Based Modeling: Overview, Validation, and Emerging Challenges & 2025 & IEEE Transactions on Artificial Intelligence & 10.1109/TAI.2025.3566362 & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[34]Generative\_AI\_Recommender\_System\_in\_E-Commerce.pdf & Microsoft Word - Nur Anis [159] -AAP & 2024 & Not independently verified (not selected) & Not independently verified (not selected) & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[35]Intelligent\_Agents\_in\_E-commerce.pdf & Intelligent Agents in E-commerce & 2000 & Not independently verified (not selected) & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[36]Light\_Trumps\_Shadow\_How\_Generative\_AI\_Agents\_Language\_Arousal\_Influences\_Users\_Interactive\_Willingness\_Evidence\_From\_Multimodal\_Analysis.pdf & Light Trumps Shadow\&\#x003F; How Generative AI Agent\&\#x2019;s Language Arousal Influences Users\&\#x2019; Interactive Willingness: Evidence From Multimodal Analysis & 2025 & IEEE Transactions on Engineering Management & 10.1109/TEM.2025.3608461 & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[37]paper\_8546.pdf & ListBERT: Learning to Rank E-commerce products with Listwise BERT & 2020 & Creator:         LaTeX with acmart 2020/11/15 v1.75 Typesetting articles for the Association for Computing Machinery and hyperref 2021-06-07 v7.00m Hypertext links for LaTeX & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[38]s44336-024-00009-2.pdf & A survey on LLM-based multi-agent systems: workflow, infrastructure, and challenges & 2024 & Vicinagearth, https://doi.org/10.1007/s44336-024-00009-2 & 10.1007/s44336-024-00009-2 & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[39]sensors-21-08448-v2.pdf & Conversational Agents: Goals, Technologies, Vision and Challenges & 2021 & sensors   Review   Conversational Agents: Goals, Technologies, Vision   and Challenges   Merav Allouch 1 , Amos Azaria 1 and Rina Azoulay 2, *   1 Computer Scie & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[3]2006.02282v3.pdf & Towards Personalized and Semantic Retrieval: An End-to-End Solution for E-commerce Search via Embedding Learning & 2020 & Not independently verified (not selected) & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[40]The\_StarCraft\_Multi-Agent\_Exploration\_Challenges\_Learning\_Multi-Stage\_Tasks\_and\_Environmental\_Factors\_Without\_Precise\_Reward\_Functions.pdf & The StarCraft Multi-Agent Exploration Challenges: Learning Multi-Stage Tasks and Environmental Factors Without Precise Reward Functions & 2023 & IEEE Access & 10.1109/ACCESS.2023.3266652 & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[41]Transforming\_E-Commerce\_AI\_Chatbots\_for\_Supercharged\_Customer\_Experiences (1).pdf & Transforming E-Commerce: AI Chatbots for Supercharged Customer Experiences & 2024 & 2024 International Conference on Information Technology Research and Innovation (ICITRI) & 10.1109/ICITRI62858.2024.10698874 & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[42]Xv2023KDD.pdf & E-commerce Search via Content Collaborative Graph Neural Network & 2023 & -  Information systems  ->  Recommender systems. & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[43]Zhou\_UniFace\_Unified\_Cross-Entropy\_Loss\_for\_Deep\_Face\_Recognition\_ICCV\_2023\_paper.pdf & UniFace: Unified Cross-Entropy Loss for Deep Face Recognition & Not independently verified & IEEE International Conference on Computer Vision & Not independently verified (not selected) & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[44]Towards\_Measuring\_Fairness\_in\_AI\_The\_Casual\_Conversations\_Dataset.pdf & Towards Measuring Fairness in AI: The Casual Conversations Dataset & 2022 & IEEE Transactions on Biometrics, Behavior, and Identity Science & 10.1109/TBIOM.2021.3132237 & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[45]TEMJournalFebruary2023\_96\_103.pdf & Facial Skin Type Prediction Based on Baumann Skin Type Solutions Theory Using Machine Learning & 2023 & TEM Journal. Volume 12, Issue 1, pages 96-103, ISSN 2217-8309, DOI: 10.18421/TEM121-13, February 2023.   Facial Skin Type Prediction Based on   Baumann Skin Typ & 10.18421/TEM121-13 & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[46]Published-version-Humanskintypeclassification.pdf & Human skin type classification using image processing and deep learning approaches & 2023 & Heliyon, 9 (2023) e21176. doi:10.1016/j.heliyon.2023.e21176 & 10.1016/j.heliyon.2023.e21176 & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[47]Skincare\_Recommendation\_System\_Based\_on\_Facial\_Ski.pdf & Skincare Recommendation System Based on Facial Skin Type with Real-Time Weather Integration & 2025 & Not independently verified (not selected) & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[48]Deep\_Learning\_Based\_Facial\_Skin\_Analysis\_and\_Product\_Recommendation.pdf & Deep Learning Based Facial Skin Analysis and Product Recommendation & 2025 & 2025 International Conference on Computing Technologies \&amp & 10.1109/ICCTDC64446.2025.11158773 & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[49]-M-Joint\_Acne\_Image\_Grading\_and\_Counting\_via\_Label\_Distribution\_Learning.pdf & Joint Acne Image Grading and Counting via Label Distribution Learning & 2019 & Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV) & 10.1109/ICCV.2019.01074 & Acne-focused AI / dermatology & Contextual acne AI evidence; less direct for the Introduction gap. & Core & ACNE04 benchmark, neighboring-grade ambiguity, LDL and joint grade/count motivation & None identified & SELECT & Directly supports a necessary Introduction claim; retained after full-text review and bibliographic verification. \\ \hline
[4]2021.naacl-industry.19.pdf & Graph-based Multilingual Product Retrieval in E-Commerce Search & 2021 & naacl 2021 & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[50]YOLOv8-QSD\_An\_Improved\_Small\_Object\_Detection\_Algorithm\_for\_Autonomous\_Vehicles\_Based\_on\_YOLOv8.pdf & YOLOv8-QSD: An Improved Small Object Detection Algorithm for Autonomous Vehicles Based on YOLOv8 & 2024 & IEEE Transactions on Instrumentation and Measurement & 10.1109/TIM.2024.3379090 & General object detection & Methodological background only; acne-specific primary studies are preferable here. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[51]YOLOv8\_A\_Novel\_Object\_Detection\_Algorithm\_with\_Enhanced\_Performance\_and\_Robustness.pdf & YOLOv8: A Novel Object Detection Algorithm with Enhanced Performance and Robustness & 2024 & 2024 International Conference on Advances in Data Engineering and Intelligent Computing Systems (ADICS) & 10.1109/ADICS58448.2024.10533619 & General object detection & Methodological background only; acne-specific primary studies are preferable here. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[52]wen-et-al-2022-acne-detection-and-severity-evaluation-with-interpretable-convolutional-neural-network-models.pdf & Acne detection and severity evaluation with interpretable convolutional neural network models & 2022 & Technology and Health Care & 10.3233/THC-228014 & Acne lesion detection/localization & Relevant to the local lesion-evidence branch and detection challenges. & Core & Interpretable lesion detection and count-based severity estimation & None identified & SELECT & Directly supports a necessary Introduction claim; retained after full-text review and bibliographic verification. \\ \hline
[53]T-YOLO\_Tiny\_Vehicle\_Detection\_Based\_on\_YOLO\_and\_Multi-Scale\_Convolutional\_Neural\_Networks.pdf & T-YOLO: Tiny Vehicle Detection Based on YOLO and Multi-Scale Convolutional Neural Networks & 2023 & IEEE Access & 10.1109/ACCESS.2021.3137638 & General object detection & Methodological background only; acne-specific primary studies are preferable here. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[54]Personalized\_Skincare\_Recommender\_System\_Using\_Deep\_Learning.pdf & Personalized Skincare Recommender System Using Deep Learning & 2025 & 2025 3rd International Conference on Advancements in Electrical, Electronics, Communication, Computing and Automation (ICAECA) & 10.1109/ICAECA63854.2025.11012227 & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[55]Optimization\_Techniques\_in\_YOLOv8\_for\_Acne\_Detection.pdf & Optimization Techniques in YOLOv8 for Acne Detection & 2025 & 2025 12th International Conference on Information Technology, Computer, and Electrical Engineering (ICITACEE) & 10.1109/ICITACEE66165.2025.11233019 & Acne lesion detection/localization & Relevant to the local lesion-evidence branch and detection challenges. & Strongly relevant & Alternative acne grading/detection evidence; reserve for deeper Related Work comparison. & None identified & DO NOT SELECT & Scientifically relevant but reserved for Related Work to avoid citation saturation in the Introduction. \\ \hline
[56]Modification\_Of\_YOLOv11n\_Algorithm\_Architecture\_to\_Improve\_Efficiency\_in\_Facial\_Acne\_Detection.pdf & Modification Of YOLOv11n Algorithm Architecture to Improve Efficiency in Facial Acne Detection & 2025 & 2025 International Conference on Information Technology and Computing (ICITCOM) & 10.1109/ICITCOM66635.2025.11265682 & Acne lesion detection/localization & Relevant to the local lesion-evidence branch and detection challenges. & Strongly relevant & Alternative acne grading/detection evidence; reserve for deeper Related Work comparison. & None identified & DO NOT SELECT & Scientifically relevant but reserved for Related Work to avoid citation saturation in the Introduction. \\ \hline
[57]Isa\_2021\_J.\_Phys.\_\_Conf.\_Ser.\_1962\_012041.pdf & Open Access proceedings Journal of Physics: Conference series & 2021 & Journal of Physics:   Conference Series   PAPER • OPEN ACCESS You may also like   - Toxicity of GO and rGO suspension   Acne Type Recognition for Mobile-Based a & Not independently verified (not selected) & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[58]Inflammatory\_Acne\_Detection\_on\_Facial\_Images\_Using\_YOLOv11\_with\_Skin\_Color\_Analysis.pdf & Inflammatory Acne Detection on Facial Images Using YOLOv11 with Skin Color Analysis & 2025 & 2025 International Conference on Data Science and Its Applications (ICoDSA) & 10.1109/ICoDSA67155.2025.11156980 & Acne lesion detection/localization & Relevant to the local lesion-evidence branch and detection challenges. & Strongly relevant & Alternative acne grading/detection evidence; reserve for deeper Related Work comparison. & None identified & DO NOT SELECT & Scientifically relevant but reserved for Related Work to avoid citation saturation in the Introduction. \\ \hline
[59]HYBRID+ATTENTION-GUIDED+CAPSULE+FRAMEWORK+FOR+AUTOMATED+FACIAL+ACNE+SEVERITY+CLASSIFICATION+(2)+(1)+(1).pdf & International Journal of Social Sciences Bulletin                                                                Volume 1, Issue 1, 2023 & 2026 & Not independently verified (not selected) & Not independently verified (not selected) & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[5]2106.09297v1.pdf & Embedding-based Product Retrieval in Taobao Search & 2021 & -  Information systems  ->  Retrieval models and ranking. & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[60]healthcare-10-02396.pdf & An Optimization-Based Technology Applied for Face Skin Symptom Detection & 2022 & Not independently verified (not selected) & Not independently verified (not selected) & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & Exact duplicate of [116]healthcare-10-02396.pdf & DO NOT SELECT & Redundant duplicate; not needed for Introduction. \\ \hline
[61]FFCA-YOLO\_for\_Small\_Object\_Detection\_in\_Remote\_Sensing\_Images.pdf & FFCA-YOLO for Small Object Detection in Remote Sensing Images & 2024 & IEEE TRANSACTIONS ON GEOSCIENCE AND REMOTE SENSING, VOL. 62, 2024 5611215   FFCA-YOLO for Small Object Detection   in Remote Sensing Images   Yin Zhang , Mu Ye & Not independently verified (not selected) & General object detection & Methodological background only; acne-specific primary studies are preferable here. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[62]Deep\_Acne\_Advancing\_Automated\_Acne\_Identification\_through\_Deep\_Neural\_Networks.pdf & Deep Acne: Advancing Automated Acne Identification through Deep Neural Networks & 2024 & 2024 1st International Conference on Advanced Computing and Emerging Technologies (ACET) & 10.1109/ACET61898.2024.10730442 & Acne-focused AI / dermatology & Contextual acne AI evidence; less direct for the Introduction gap. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[63]biomedinformatics-04-00059-v4.pdf & RETRACTED: Utilizing Generative Adversarial Networks for Acne Dataset Generation in Dermatology & 2024 & Not independently verified (not selected) & Not independently verified (not selected) & Acne-focused AI / dermatology & Contextual acne AI evidence; less direct for the Introduction gap. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[64]Automatic\_Acne\_Detection\_Model\_Based\_on\_Improved\_YOLOv7.pdf & Automatic Acne Detection Model Based on Improved YOLOv7 & 2024 & IEEE Access & 10.1109/ACCESS.2024.3520641 & Acne lesion detection/localization & Relevant to the local lesion-evidence branch and detection challenges. & Strongly relevant & Alternative acne grading/detection evidence; reserve for deeper Related Work comparison. & None identified & DO NOT SELECT & Scientifically relevant but reserved for Related Work to avoid citation saturation in the Introduction. \\ \hline
[65]Acne\_Detection\_and\_Facial\_Skin\_Severity\_Classification\_into\_Four\_Categories\_Using\_You\_Only\_Look\_Once\_YOLO\_V11.pdf & Acne Detection and Facial Skin Severity Classification into Four Categories Using You Only Look Once (YOLO) V11 & 2025 & 2025 International Seminar on Application for Technology of Information and Communication (iSemantic) & 10.1109/ISemantic67418.2025.11291986 & Acne severity grading / lesion-aware assessment & Directly relevant to ordinal grading, lesion burden, or evaluation. & Strongly relevant & Alternative acne grading/detection evidence; reserve for deeper Related Work comparison. & None identified & DO NOT SELECT & Scientifically relevant but reserved for Related Work to avoid citation saturation in the Introduction. \\ \hline
[66]A\_Comparative\_Study\_on\_Automated\_Detection\_of\_Skin\_Diseases\_Using\_Various\_Image\_Segmentation\_and\_Deep\_Learning\_Approaches.pdf & A Comparative Study on Automated Detection of Skin Diseases Using Various Image Segmentation and Deep Learning Approaches & 2024 & 2024 IEEE International Conference on Control \&amp & 10.1109/CERIA64726.2024.10914766 & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[67]38285-1273-31375-1-10-20251114.pdf & ClearFace: Facial Acne Detection and Classification System Using YOLOv11 and EfficientNet-B0 & 2025 & Not independently verified (not selected) & Not independently verified (not selected) & Acne lesion detection/localization & Relevant to the local lesion-evidence branch and detection challenges. & Strongly relevant & Alternative acne grading/detection evidence; reserve for deeper Related Work comparison. & None identified & DO NOT SELECT & Scientifically relevant but reserved for Related Work to avoid citation saturation in the Introduction. \\ \hline
[68]-M-sensors-22-06828.pdf & Acne Detection by Ensemble Neural Networks & 2022 & sensors   Article   Acne Detection by Ensemble Neural Networks   Hang Zhang 1, * and Tianyi Ma 2   1 School of Materials Science and Engineering, Nanyang Techno & Not independently verified (not selected) & Acne lesion detection/localization & Relevant to the local lesion-evidence branch and detection challenges. & Strongly relevant & Alternative acne grading/detection evidence; reserve for deeper Related Work comparison. & None identified & DO NOT SELECT & Scientifically relevant but reserved for Related Work to avoid citation saturation in the Introduction. \\ \hline
[69]diagnostics-12-01879.pdf & Automatic Acne Object Detection and Acne Severity Grading Using Smartphone Images and Artificial Intelligence & 2022 & Diagnostics & 10.3390/diagnostics12081879 & Acne severity grading / lesion-aware assessment & Directly relevant to ordinal grading, lesion burden, or evaluation. & Core & Detector-derived lesion counts used for severity grading; class imbalance & None identified & SELECT & Directly supports a necessary Introduction claim; retained after full-text review and bibliographic verification. \\ \hline
[6]2202.05317v2.pdf & A Multi-task Learning Framework for Product Ranking with BERT & 2022 & -  Computing methodologies  ->  Multi-task learning.-  Information systems  ->  Retrieval models and ranking. & Not independently verified (not selected) & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[70]-M-2216\_paper.pdf & AcneAI: A New Acne Severity Assessment Method Using Digital Images and Deep Learning & 2024 & Medical Image Computing and Computer Assisted Intervention -- MICCAI 2024, LNCS 15005 & 10.1007/978-3-031-72086-4\_7 & Acne-focused AI / dermatology & Contextual acne AI evidence; less direct for the Introduction gap. & Core & Lesion-level segmentation/scoring aggregated to global severity & Prepublication/author manuscript; bibliographic record normalized to MICCAI 2024 published chapter. & SELECT & Directly supports a necessary Introduction claim; retained after full-text review and bibliographic verification. \\ \hline
[71]-M\_An experimental evaluation of deep learning-based models for acne severity classification in humans.pdf & An experimental evaluation of deep learning-based models for acne severity classification in humans & 2025 & Connection Science & 10.1080/09540091.2025.2533867 & Acne severity grading / lesion-aware assessment & Directly relevant to ordinal grading, lesion burden, or evaluation. & Core & Recent comparative deep-learning acne-severity classification & None identified & SELECT & Directly supports a necessary Introduction claim; retained after full-text review and bibliographic verification. \\ \hline
[72]-M-2403.00268v1.pdf & Improving Acne Image Grading with Label Distribution Smoothing & 2024 & 2024 IEEE International Symposium on Biomedical Imaging (ISBI) & 10.1109/ISBI56570.2024.10635668 & Acne-focused AI / dermatology & Contextual acne AI evidence; less direct for the Introduction gap. & Core & Ordinal label uncertainty and severity-aware smoothing & arXiv v1; bibliographic record normalized to peer-reviewed ISBI 2024 version. & SELECT & Directly supports a necessary Introduction claim; retained after full-text review and bibliographic verification. \\ \hline
[73]-M-Skin Research and Technology - 2022 - Liu - AcneGrader  An ensemble pruning of the deep learning base models to grade acne.pdf & AcneGrader: An ensemble pruning of the deep learning base models to grade acne & 2022 & Skin Research and Technology & 10.1111/srt.13166 & Acne severity grading / lesion-aware assessment & Directly relevant to ordinal grading, lesion burden, or evaluation. & Core & Ensemble-based grading and computational redundancy & None identified & SELECT & Directly supports a necessary Introduction claim; retained after full-text review and bibliographic verification. \\ \hline
[74]-M-bioengineering-12-00342.pdf & Feature Feedback-Based Pseudo-Label Learning for Multi-Standards in Clinical Acne Grading & 2025 & Bioengineering & 10.3390/bioengineering12040342 & Acne severity grading / lesion-aware assessment & Directly relevant to ordinal grading, lesion burden, or evaluation. & Core & Feature-feedback/pseudo-label training and external-dataset context & None identified & SELECT & Directly supports a necessary Introduction claim; retained after full-text review and bibliographic verification. \\ \hline
[75]-M-KIEGLFNAunifiedacnegradingframeworkonfaceimages.pdf & KIEGLFN: A unified acne grading framework on face images & 2022 & Computer Methods and Programs in Biomedicine & 10.1016/j.cmpb.2022.106911 & Acne severity grading / lesion-aware assessment & Directly relevant to ordinal grading, lesion burden, or evaluation. & Core & Global--local acne representation and complementary local/global evidence & None identified & SELECT & Directly supports a necessary Introduction claim; retained after full-text review and bibliographic verification. \\ \hline
[76]Studies\_on\_Different\_CNN\_Algorithms\_for\_Face\_Skin\_Disease\_Classification\_Based\_on\_Clinical\_Images.pdf & Studies on Different CNN Algorithms for Face Skin Disease Classification Based on Clinical Images & 2019 & IEEE Access & 10.1109/ACCESS.2019.2918221 & Dermatology AI / skin-image analysis & Provides broad reliability or medical-image context but is not acne-grading specific. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[77]Multiclass\_Classification\_of\_Facial\_Skin\_Spot\_with\_CNN\_Architecture.pdf & Multiclass Classification of Facial Skin Spot with CNN Architecture & 2025 & 2025 9th International Conference on Electrical, Telecommunication and Computer Engineering (ELTICOM) & 10.1109/ELTICOM67568.2025.11336045 & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[78]Mi\_Privacy-Preserving\_Face\_Recognition\_Using\_Random\_Frequency\_Components\_ICCV\_2023\_paper.pdf & Privacy-Preserving Face Recognition Using Random Frequency Components & Not independently verified & IEEE International Conference on Computer Vision & Not independently verified (not selected) & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[79]Meta\_Balanced\_Network\_for\_Fair\_Face\_Recognition.pdf & Meta Balanced Network for Fair Face Recognition & 2022 & IEEE Transactions on Pattern Analysis and Machine Intelligence & 10.1109/TPAMI.2021.3103191 & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[7]2307.04322v1.pdf & Graph Contrastive Learning with Multi-Objective for Personalized Product Retrieval in Taobao Search & 2023 & Not independently verified (not selected) & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[80]main.pdf & PLFace: Progressive Learning for Face Recognition with Mask Bias & 2023 & Pattern Recognition, 135 (2023) 109142. doi:10.1016/j.patcog.2022.109142 & 10.1016/j.patcog.2022.109142 & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[81]Li\_Rethinking\_Feature-Based\_Knowledge\_Distillation\_for\_Face\_Recognition\_CVPR\_2023\_paper.pdf & Rethinking Feature-Based Knowledge Distillation for Face Recognition & Not independently verified & IEEE Conference on Computer Vision and Pattern Recognition & Not independently verified (not selected) & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[82]Kim\_KeyPoint\_Relative\_Position\_Encoding\_for\_Face\_Recognition\_CVPR\_2024\_paper.pdf & KeyPoint Relative Position Encoding for Face Recognition & Not independently verified & IEEE Conference on Computer Vision and Pattern Recognition & Not independently verified (not selected) & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[83]Kim\_AdaFace\_Quality\_Adaptive\_Margin\_for\_Face\_Recognition\_CVPR\_2022\_paper.pdf & AdaFace: Quality Adaptive Margin for Face Recognition & Not independently verified & IEEE Conference on Computer Vision and Pattern Recognition & Not independently verified (not selected) & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[84]Improving\_Gender\_Classification\_based\_on\_Skin\_Color\_using\_CNN\_Transfer\_Learning.pdf & Improving Gender Classification based on Skin Color using CNN Transfer Learning & 2022 & 2022 3rd International Conference on Artificial Intelligence and Data Sciences (AiDAS) & 10.1109/AiDAS56890.2022.9918791 & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[85]IJEEE-V11I11P1251.pdf & A Fine Tune CNN Model for Human Skin Type Classification & 2024 & SSRG International Journal of Electrical and Electronics Engineering Volume 11 Issue 11, 264-274, November 2024   ISSN: 2348-8379/ https://doi.org/10.14445/2348 & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[86]GhostFaceNets\_Lightweight\_Face\_Recognition\_Model\_From\_Cheap\_Operations.pdf & GhostFaceNets: Lightweight Face Recognition Model From Cheap Operations & 2023 & Not independently verified (not selected) & Not independently verified (not selected) & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[87]3D\_face\_recognition\_A\_comprehensive\_survey\_in\_2022.pdf & 3D face recognition: A comprehensive survey in 2022 & 2023 & Not independently verified (not selected) & Not independently verified (not selected) & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[88]2023.I2.004.pdf & Facial Skin Type Detection for Race Classification using Convolutional Neural Network and Haar Cascade Method & 2023 & Not independently verified (not selected) & Not independently verified (not selected) & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[89]2305.01021v1.pdf & Synthetic Data for Face Recognition: Current State and Future Prospects & 2023 & Not independently verified (not selected) & arXiv:2305.01021v1 & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[8]2307.07924v5.pdf & ChatDev: Communicative Agents for Software Development & 2024 & Not independently verified (not selected) & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[90]2307.01838v2.pdf & EdgeFace: Efficient Face Recognition Model for Edge Devices & 2015 & JOURNAL OF LATEX CLASS FILES, VOL. 14, NO. 8, AUGUST 2015 1   EdgeFace : Efficient Face Recognition Model   for Edge Devices   Anjith George, Member, IEEE, Chri & Not independently verified (not selected) & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[91]2404.04580v2.pdf & SDFR: Synthetic Data for Face Recognition Competition & 2024 & Not independently verified (not selected) & Not independently verified (not selected) & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[92]12831-Article Text-14293-1-10-20230921.pdf & Comparative Analysis of CNN and CNN-SVM Methods For Classification Types of Human Skin Disease & 2023 & Not independently verified (not selected) & Not independently verified (not selected) & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[93]3472810.pdf & Age-Invariant Face Recognition by Multi-Feature Fusionand Decomposition with Self-attention & 2022 & ACM Trans. Multimedia Comput. Commun. Appl. 2022.18:1-18 & Not independently verified (not selected) & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[94]3673224.pdf & Toward a Privacy-Preserving Face Recognition System: A Survey of Leakages and Solutions & 2025 & ACM Comput. Surv. 2025.57:1-38 & Not independently verified (not selected) & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[95]A novel DeepMaskNet model for face mask detection and masked facial recognition.pdf & A novel DeepMaskNet model for face mask detection and masked facial recognition & 2022 & Journal of King Saud University - Computer and Information Sciences, 34 (2022) 9905-9914. doi:10.1016/j.jksuci.2021.12.017 & 10.1016/j.jksuci.2021.12.017 & Other / peripheral topic & Does not directly support the focused CG-HAF Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[96]Advancing\_Skin\_Type\_Classification\_The\_Development\_of\_Malaysian\_Facial\_Skin\_Texture\_Datasets\_for\_Machine\_Learning.pdf & Advancing Skin Type Classification: The Development of Malaysian Facial Skin Texture Datasets for Machine Learning & 2025 & 2025 IEEE 15th Symposium on Computer Applications \&amp & 10.1109/ISCAIE64985.2025.11080992 & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[97]Bae\_DigiFace-1M\_1\_Million\_Digital\_Face\_Images\_for\_Face\_Recognition\_WACV\_2023\_paper.pdf & DigiFace-1M: 1 Million Digital Face Images for Face Recognition & Not independently verified & IEEE Winter Conference on Applications of Computer Vision & Not independently verified (not selected) & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[98]Boutros\_ElasticFace\_Elastic\_Margin\_Loss\_for\_Deep\_Face\_Recognition\_CVPRW\_2022\_paper.pdf & ElasticFace: Elastic Margin Loss for Deep Face Recognition & Not independently verified & IEEE Conference on Computer Vision and Pattern Recognition Workshops & Not independently verified (not selected) & Face recognition / face analysis & Peripheral computer-vision context; not needed for acne-severity Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
[99]Cosmetic\_Skin\_Type\_Classification\_Using\_CNN\_With\_Product\_Recommendation.pdf & Cosmetic Skin Type Classification Using CNN With Product Recommendation & 2021 & 2021 12th International Conference on Computing Communication and Networking Technologies (ICCCNT) & 10.1109/ICCCNT51525.2021.9580174 & Facial-skin / cosmetic AI & Adjacent skincare context; not needed for focused CG-HAF Introduction. & Contextual & Broader methodological, dermatology-AI, or skin-analysis context if later needed. & None identified & DO NOT SELECT & Contextual but weaker than selected acne-specific primary evidence for this Introduction. \\ \hline
[9]2308.00352v7.pdf & MetaGPT: Meta Programming for A Multi-Agent Collaborative Framework & 2024 & Not independently verified (not selected) & Not independently verified (not selected) & Agentic AI / e-commerce / recommendation & Relevant to broader SkinAgent project, not the CG-HAF methodological Introduction. & Not suitable for Introduction & No necessary claim in the focused CG-HAF Introduction. & None identified & DO NOT SELECT & Outside the focused methodological scope of the CG-HAF Introduction. \\ \hline
jpm-15-00238-v2.pdf & Artificial Intelligence in the Assessment and Grading of Acne Vulgaris: A Systematic Review & 2025 & Journal of Personalized Medicine & 10.3390/jpm15060238 & Acne-focused AI / dermatology & Contextual acne AI evidence; less direct for the Introduction gap. & Core & Global grading vs lesion counting; validation/generalization limitations & None identified & SELECT & Directly supports a necessary Introduction claim; retained after full-text review and bibliographic verification. \\ \hline
technologies-14-00116-v2.pdf & A Study of SimCLR-Based Self-Supervised Learning for Acne Severity Grading Under Label-Scarce Conditions & 2026 & Technologies & 10.3390/technologies14020116 & Acne severity grading / lesion-aware assessment & Directly relevant to ordinal grading, lesion burden, or evaluation. & Core & Ordinal metrics, localized cues, controlled acne-grading evaluation & None identified & SELECT & Directly supports a necessary Introduction claim; retained after full-text review and bibliographic verification. \\ \hline
\end{longtable}
\end{landscape}


\section*{References Used in the Introduction}
[1] X. Wu, N. Wen, J. Liang, Y.-K. Lai, D. She, M.-M. Cheng, and J. Yang, ``Joint Acne Image Grading and Counting via Label Distribution Learning,'' in Proc. IEEE/CVF Int. Conf. Comput. Vis. (ICCV), 2019, pp. 10641--10650, doi: 10.1109/ICCV.2019.01074.

[2] D. O. Traini, G. Palmisano, C. Guerriero, and K. Peris, ``Artificial Intelligence in the Assessment and Grading of Acne Vulgaris: A Systematic Review,'' J. Pers. Med., vol. 15, no. 6, Art. no. 238, 2025, doi: 10.3390/jpm15060238.

[3] K. Prokhorov and A. A. Kalinin, ``Improving Acne Image Grading with Label Distribution Smoothing,'' in Proc. 2024 IEEE Int. Symp. Biomed. Imaging (ISBI), 2024, pp. 1--5, doi: 10.1109/ISBI56570.2024.10635668.

[4] Y. Lin, J. Jiang, Z. Ma, D. Chen, Y. Guan, H. You, X. Cheng, B. Liu, and G. Luo, ``KIEGLFN: A unified acne grading framework on face images,'' Comput. Methods Programs Biomed., vol. 221, Art. no. 106911, 2022, doi: 10.1016/j.cmpb.2022.106911.

[5] Y. Lin, J. Jiang, D. Chen, Z. Ma, Y. Guan, X. Liu, H. You, and J. Yang, ``DED: Diagnostic Evidence Distillation for acne severity grading on face images,'' Expert Syst. Appl., vol. 228, Art. no. 120312, 2023, doi: 10.1016/j.eswa.2023.120312.

[6] Q. T. Huynh, P. H. Nguyen, H. X. Le, L. T. Ngo, N.-T. Trinh, M. T.-T. Tran, H. T. Nguyen, N. T. Vu, A. T. Nguyen, K. Suda, K. Tsuji, T. Ishii, T. X. Ngo, and H. T. Ngo, ``Automatic Acne Object Detection and Acne Severity Grading Using Smartphone Images and Artificial Intelligence,'' Diagnostics, vol. 12, no. 8, Art. no. 1879, 2022, doi: 10.3390/diagnostics12081879.

[7] H. Wen, W. Yu, Y. Wu, J. Zhao, X. Liu, Z. Kuang, and R. Fan, ``Acne detection and severity evaluation with interpretable convolutional neural network models,'' Technol. Health Care, vol. 30, suppl. 1, pp. S143--S153, 2022, doi: 10.3233/THC-228014.

[8] K. Min, G.-H. Lee, and S.-W. Lee, ``ACNet: Mask-Aware Attention with Dynamic Context Enhancement for Robust Acne Detection,'' in Proc. 2021 IEEE Int. Conf. Syst., Man, Cybern. (SMC), 2021, pp. 2724--2729, doi: 10.1109/SMC52423.2021.9659243.

[9] S. Liu, Y. Fan, M. Duan, Y. Wang, G. Su, Y. Ren, L. Huang, and F. Zhou, ``AcneGrader: An ensemble pruning of the deep learning base models to grade acne,'' Skin Res. Technol., vol. 28, no. 5, pp. 677--688, 2022, doi: 10.1111/srt.13166.

[10] Y. Lin, J. Jiang, D. Chen, Z. Ma, Y. Guan, X. Liu, H. You, J. Yang, and X. Cheng, ``Acne Severity Grading on Face Images via Extraction and Guidance of Prior Knowledge,'' in Proc. 2022 IEEE Int. Conf. Bioinformatics Biomed. (BIBM), 2022, pp. 1639--1643, doi: 10.1109/BIBM55620.2022.9995101.

[11] Y.-Y. Chen, H.-T. Chan, H.-C. Wang, C.-S. Wang, H.-H. Chen, P.-H. Chen, Y.-J. Chen, S.-H. Hsu, and C.-H. Hsia, ``Feature Feedback-Based Pseudo-Label Learning for Multi-Standards in Clinical Acne Grading,'' Bioengineering, vol. 12, no. 4, Art. no. 342, 2025, doi: 10.3390/bioengineering12040342.

[12] L. Gazeau, H. Nguyen, Z. Nguyen, M. Lebedeva, T. Nguyen, T.-D. To, J. Le Digabel, J. Filiol, G. Josse, C. Perlis, and J. Wolfe, ``AcneAI: A New Acne Severity Assessment Method Using Digital Images and Deep Learning,'' in Medical Image Computing and Computer Assisted Intervention -- MICCAI 2024, LNCS, vol. 15005, 2024, pp. 68--78, doi: 10.1007/978-3-031-72086-4\_7.

[13] K. Srijiranon, N. Varisthanist, and T. Tanantong, ``A Study of SimCLR-Based Self-Supervised Learning for Acne Severity Grading Under Label-Scarce Conditions,'' Technologies, vol. 14, no. 2, Art. no. 116, 2026, doi: 10.3390/technologies14020116.

[14] A. Shaik, J. J. Kanichai, A. B. Kurumthottam, V. Garg, and B. Ananthakrishnan, ``An experimental evaluation of deep learning-based models for acne severity classification in humans,'' Connection Sci., vol. 37, no. 1, Art. no. 2533867, 2025, doi: 10.1080/09540091.2025.2533867.


==> sections/declarations_template.tex <==
% -----------------------------------------------------------------------------
% TEMPLATE ONLY — complete with verified author/project information before use.
% Add \input{sections/declarations_template} in main.tex only after completion.
% -----------------------------------------------------------------------------
\section*{CRediT authorship contribution statement}
[TO COMPLETE: use verified author names and contribution roles only.]

\section*{Funding}
[TO COMPLETE: provide verified funding information, or the journal-appropriate no-funding statement.]

\section*{Declaration of competing interest}
[TO COMPLETE: provide the verified competing-interest declaration.]

\section*{Data availability}
ACNE04 is the benchmark used in this study. [TO COMPLETE: add the verified access/citation statement and specify which derived prediction/statistical artifacts, if any, will be shared.]

\section*{Code availability}
[TO COMPLETE: state the verified code/reproducibility-material availability. Do not promise public release unless approved by all authors.]

\section*{Acknowledgements}
[OPTIONAL — TO COMPLETE OR DELETE.]

\section*{Declaration of generative AI and AI-assisted technologies in manuscript preparation}
[TO COMPLETE in the form required by the journal/publisher, if applicable. State the tool(s), the purpose of use, and that the authors reviewed and take responsibility for the final content.]

